Source-free Video Domain Adaptation by Learning from Noisy Labels

Despite the progress seen in classification methods, current approaches for handling videos with distribution shifts in source and target domains remain source-dependent as they require access to the source data during the adaptation stage. In this paper, we present a self-training based source-free video domain adaptation approach to address this challenge by bridging the gap between the source and the target domains. We use the source pre-trained model to generate pseudo-labels for the target domain samples, which are inevitably noisy. Thus, we treat the problem of source-free video domain adaptation as learning from noisy labels and argue that the samples with correct pseudo-labels can help us in adaptation. To this end, we leverage the cross-entropy loss as an indicator of the correctness of the pseudo-labels and use the resulting small-loss samples from the target domain for fine-tuning the model. We further enhance the adaptation performance by implementing a teacher-student (TS) framework, in which the teacher, which is updated gradually, produces reliable pseudo-labels. Meanwhile, the student undergoes fine-tuning on the target domain videos using these generated pseudo-labels to improve its performance. Extensive experimental evaluations show that our methods, termed as CleanAdapt, CleanAdapt + TS, achieve state-of-the-art results, outperforming the existing approaches on various open datasets. Our source code is publicly available at https://avijit9.github.io/CleanAdapt.

==> assets/tables/epic-additional.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table*}[htp]
% \scriptsize
\centering
\caption{Performance comparisons with state-of-the-art video domain adaptation methods on EPIC-Kitchens dataset. All models reported are single-stream (appearance) networks. The results for our methods are highlighted in \textcolor{gray}{gray} color.}

\begin{tabular}{cclllllll}
\hline
 \textbf{Method} & \textbf{Source-free?} &\textbf{D2$\rightarrow$D1} & \textbf{D3$\rightarrow$D1} & \textbf{D1$\rightarrow$D2} & \textbf{D3$\rightarrow$D2} & \textbf{D1$\rightarrow$D3} & \textbf{D2$\rightarrow$D3} & \textbf{Mean}   \\ \hline 
Source only & &  35.4 &  34.6 &32.8  & 35.8&34.1  &39.1  & 35.3 \\ 

DANN~\cite{ganin2015unsupervised} & \textcolor{red}{\xmark}& 38.3 & 38.8 & 37.7 & 42.1&36.6 &41.9 &39.2\\

ADDA~\cite{tzeng2017adversarial} &\textcolor{red}{\xmark} & 36.3  & 36.1 & 35.4 & 41.4& 34.9& 40.8&37.4 \\

TA3N~\cite{chen2019temporal} &\textcolor{red}{\xmark} & 40.9& 39.9&34.2 &44.2 &37.4 &42.8 & 39.9 \\

CoMix~\cite{sahoo2021contrast}  &\textcolor{red}{\xmark} & 38.6 &42.3 & 42.9 &49.2 &40.9 &45.2 &43.2 \\ 

 Target Supervised& & 57.0 & 57.0 & 64.0 & 64.0 & 63.7 & 63.7   & 61.5\\ \hline
 
 \rowcolor{Gray}
 Source only & & 40.9 & 38.6 & 39.3 & 41.3 & 37.3 & 42.4 & 39.9 \\ \rowcolor{Gray}
 \method{} & \textcolor{green}{\cmark} &  44.6 \textcolor{ForestGreen}{$\blacktriangle \text{+} 3.7$}& 40.7 \textcolor{ForestGreen}{$\blacktriangle \text{+}2.1$ } &  44.5 \textcolor{ForestGreen}{$\blacktriangle \text{+} 5.2$} &  47.1 \textcolor{ForestGreen}{$\blacktriangle \text{+}5.8$ }&  40.9 \textcolor{ForestGreen}{$\blacktriangle \text{+}3.6$ } & 45.7 \textcolor{ForestGreen}{$\blacktriangle \text{+}3.3$}&  43.9 \textcolor{ForestGreen}{$\blacktriangle \text{+} 4.0$}  \\ \rowcolor{Gray}
 Target Supervised & & 60.5 & 60.5 & 68.4  & 68.4 & 68.8  & 68.8  &  65.9 \\ \hline
\end{tabular}
\label{tab:epic-additional}
% \vspace{-0.6cm}
\end{table*}

==> assets/tables/retrieval-additional-uh.tex <==
\begin{table}[h!]
\centering
\scriptsize
\caption{Cross-domain video retrieval results on UCF $\leftrightarrow$ HMDB dataset. Given queries from the target domain, we evaluate retrieved videos from the source domain in terms of R@k, where $k \in \{1, 5, 10\}$. Note that, all models reported here are single-steam (appearance only) networks.}
\begin{tabular}{@{}lrrrrrr@{}}
\toprule

{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{3}{c}{\textbf{UCF $\rightarrow$ HMDB}} & \multicolumn{3}{c}{\textbf{HMDB $\rightarrow$ UCF}}\\

\cmidrule(lr){2-4}\cmidrule(l){5-7}

\multicolumn{1}{c}{} & \multicolumn{1}{c}{R@1} & \multicolumn{1}{c}{R@5} & \multicolumn{1}{c}{R@10} & \multicolumn{1}{c}{R@1} & R@5 & \multicolumn{1}{c}{R@10} \\

\midrule

Source Only & 0.81 & 0.86 & \textbf{0.89} & 0.87 & 0.92  & 0.94 \\

\method{} & \textbf{0.83} & \textbf{0.87} & 0.88 & \textbf{0.89} & \textbf{0.94}  & \textbf{0.96} \\
\bottomrule
\end{tabular}
\label{tab:uh-retrieval-additional}
\end{table}


\setlength{\textfloatsep}{0.3cm}


% \begin{table}[h!]

% \centering
% \caption{Comparison with state-of-the-art image based source-free domain adaptation techniques.}
% \begin{adjustbox}{max width=0.9\columnwidth}
% \begin{tabular}{lccccc}
% \hline
% %\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{} & \multicolumn{4}{c}{\textbf{Datasets}} \\ \cline{3-6} 
% {\textbf{Method}} &  &  \textbf{UCF $\rightarrow$ HMDB} &  & \textbf{HMDB $\rightarrow$ UCF}  &  \\ \hline

% Source only & & 80.6 & & 89.3 & \\
% Yang \etal~\cite{yang2021exploiting} & & \textbf{86.6} & & 91.4 & \\
% Liang \etal~\cite{liang2020we} & & 82.5 & & 91.9 & \\
% CleanAdapt & & 86.1 & & \textbf{96.1} & \\
% Target supervised & & 93.6 & &  98.4 & \\ \hline
% \end{tabular}
% \end{adjustbox}
% \label{tab:source-free}
% \end{table}

==> assets/tables/retrieval-additional.tex <==




\begin{table*}[ht!]
\centering
\caption{Cross-domain video retrieval results on EPIC-Kitchens dataset. Given queries from the target domain, we evaluate retrieved videos from the source domain in terms of R@k, where $k \in \{1, 5, 10\}$. Note that, all models reported here are single-steam (appearance only) networks.}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{@{}lrrrrrrrrrrrrrrrrrr@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{3}{c}{\textbf{D2 $\rightarrow$ D1 }} & \multicolumn{3}{c}{\textbf{D3 $\rightarrow$ D1}}   & \multicolumn{3}{c}{\textbf{D1 $\rightarrow$ D2}}   &  \multicolumn{3}{c}{\textbf{D3 $\rightarrow$ D2}}&

\multicolumn{3}{c}{\textbf{D1 $\rightarrow$ D3}}& \multicolumn{3}{c}{\textbf{D2 $\rightarrow$ D3}}\\

\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}\cmidrule(lr){14-16}\cmidrule(l){17-19}

\multicolumn{1}{c}{} & \multicolumn{1}{c}{R@1} & \multicolumn{1}{c}{R@5} & \multicolumn{1}{c}{R@10} & \multicolumn{1}{c}{R@1} & R@5 & \multicolumn{1}{c}{R@10}& \multicolumn{1}{c}{R@1} & \multicolumn{1}{c}{R@5} & \multicolumn{1}{c}{R@10} & \multicolumn{1}{c}{R@1} & \multicolumn{1}{c}{R@5} & \multicolumn{1}{c}{R@10} &\multicolumn{1}{c}{R@1} & \multicolumn{1}{c}{R@5} & \multicolumn{1}{c}{R@10} &\multicolumn{1}{c}{R@1} & \multicolumn{1}{c}{R@5} & \multicolumn{1}{c}{R@10}\\\midrule

Source only & \textbf{0.39} & 0.64 &0.77 & 0.27 &\textbf{0.66} & \textbf{0.77} & \textbf{0.34} & 0.68 & \textbf{0.84} & 0.38 & 0.71 & 0.82& 0.32&0.68&0.80& 0.36 &0.68 &\textbf{0.82}  \\
\method{} & 0.37 & \textbf{0.69} & \textbf{0.79}&  \textbf{0.31}&0.64 &\textbf{0.77} & \textbf{0.34} & \textbf{0.69 }& 0.82 & \textbf{0.39} & \textbf{0.74} & \textbf{0.83} & \textbf{0.34} &\textbf{0.68}&\textbf{0.81}&\textbf{0.40} &\textbf{0.70} &\textbf{0.82 }\\ 
\bottomrule
           
\end{tabular}}
\label{tab:epic-retrieval-additional}
\vspace{-0.1cm}
\end{table*}


% \setlength{\textfloatsep}{0.3cm}


% \begin{figure}
%      \centering
%      \begin{subfigure}[b]{0.9\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{assets/d2-d1-rgb.png}
%          \caption*{}
%          \label{fig:y equals x}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.88\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{assets/d2-d3-rgb.png}
%          \caption*{}
%          \label{fig:three sin x}
%      \end{subfigure}
%      \hfill
     
%         \caption{}
%         \label{fig:three graphs}
% \end{figure}



==> assets/tables/source-free.tex <==
\begin{table}[h!]

\centering
\caption{Comparison with state-of-the-art image-based source-free domain adaptation techniques.}
\begin{adjustbox}{max width=0.9\columnwidth}
\begin{tabular}{lccccccc}
\hline
%\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{} & \multicolumn{4}{c}{\textbf{Datasets}} \\ \cline{3-6} 
{\textbf{Method}} & \textbf{Backbone} & &  &  \textbf{UCF $\rightarrow$ HMDB} &  & \textbf{HMDB $\rightarrow$ UCF}  &  \\ \hline

Source only & TRN & & & 72.7 & & 72.2& \\
Kim \etal~\cite{kim2021domain} & TRN & & & 69.9 & & 74.9  & \\

Li \etal~\cite{li2020model} & TRN & & & 74.4 & & 67.3  & \\
Yang \etal~\cite{yang2020unsupervised} & TRN & & & 75.3 & & 76.3  & \\
Qiu \etal~\cite{qiu2021source}& TRN & & & 75.8 & & 68.2  &
\\\hline


Source only & I3D & & & 80.6 & & 89.3 & \\
Yang \etal~\cite{yang2021exploiting} & I3D & & & 86.6 & & 91.4 & \\
Liang \etal~\cite{liang2020we} & I3D & & & 82.5 & & 91.9 & \\
\method{} & I3D & & & 86.1 & & 96.1 & \\
\methodj{} & I3D & & & \textbf{88.6} & & \textbf{96.7} & \\\hline
% Target supervised & & & & 93.6 & &  98.4 & \\ \hline
\end{tabular}
\end{adjustbox}
\label{tab:source-free}
\end{table}


==> assets/tables/ucfsmall-hmdbsmall.tex <==
\begin{table}[ht!]

\centering
\caption{Performance comparisons with state-of-the-art video domain adaptation methods on UCF  $\leftrightarrow$ HMDB\textsubscript{small}.}
\begin{adjustbox}{max width=0.9\columnwidth}
\begin{tabular}{lccccccc}
\hline
%\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{} & \multicolumn{4}{c}{\textbf{Datasets}} \\ \cline{3-6} 
{\textbf{Method}} &  &  &  \textbf{UCF $\rightarrow$ HMDB} &  & \textbf{HMDB $\rightarrow$ UCF}  &  \\ \hline

Source only  & & & 97.3 & & 96.8& \\
SHOT~\cite{liang2020we} & & & 99.3 & & 99.5& \\
3C-GAN~\cite{li2020model} & & & 98.3 & & 99.5& \\
SFDA~\cite{kim2021domain} & & & 98.0 & & 99.3& \\
HCL~\cite{huang2021model}& & & 99.3 & & 99.5& \\
MTRAN~\cite{huang2022relative} & & & 100 & & 100& \\
\hline
Source only  & & & 98.3 & & 97.8& \\
\methodj{} & & & 100 & & 100& \\
Target Supervised  & & & 100 & & 100  &\\
\hline
\end{tabular}
\end{adjustbox}
\label{tab:uh-small}

\end{table}
